Diverse Controllable Diffusion Policy with Signal Temporal Logic

Generating realistic simulations is critical for autonomous system applications such as self-driving and human-robot interactions. However, driving simulators nowadays still have difficulty in generating controllable, diverse, and rule-compliant behaviors for road participants: Rule-based models cannot produce diverse behaviors and require careful tuning, whereas learning-based methods imitate the policy from data but are not designed to follow the rules explicitly. Besides, the real-world datasets are by nature "single-outcome", making the learning method hard to generate diverse behaviors. In this paper, we leverage Signal Temporal Logic (STL) and Diffusion Models to learn controllable, diverse, and rule-aware policy. We first calibrate the STL on the real-world data, then generate diverse synthetic data using trajectory optimization, and finally learn the rectified diffusion policy on the augmented dataset. We test on the NuScenes dataset and our approach can achieve the most diverse rule-compliant trajectories compared to other baselines, with a runtime 1/17X to the second-best approach. In the closed-loop testing, our approach reaches the highest diversity, rule satisfaction rate, and the least collision rate. Our method can generate varied characteristics conditional on different STL parameters in testing. A case study on human-robot encounter scenarios shows our approach can generate diverse and closed-to-oracle trajectories. The annotation tool, augmented dataset, and code are available at https://github.com/mengyuest/pSTL-diffusion-policy.

==> rebuttal/zz_post_acceptance.tex <==
\newpage
\onecolumn

\setcounter{equation}{0}
\setcounter{section}{0}
\titleformat{\section}{\large\raggedright}{\thesection}{1em}{}
\begin{center}
\LARGE{Statement of changes}
\end{center}

% \doublespacing
\linespread{2}

\vspace{2em}

% \red{make it spreaded}
We thank all reviewers and the editor of IEEE Robotics and Automation Letters (RA-L) for accepting our paper. This additional material addresses the remaining issues from the editor and the reviewers and reflects the changes in the manuscript. The updated content in the manuscript is written in \pac{``Magenta"}, and the changes from the previous review are written in \rbt{``Teal"}. We appreciate your effort throughout the whole review process.


\section{Responses to the editor}
Thank you for the conditional acceptance of our manuscript. We have addressed the concerns raised by Reviewer 6 in both this statement and the updated manuscript. 

Regarding the windowed diffusion-based controllers (such as Diffusion Policy [1]), we agree that it is necessary to reference them, and we updated Sec.~\ref{sec:intro} and Sec.~\ref{sec:related} accordingly. The reasons we didn't mention it in the initial submission are: (1) they do not explicitly address trajectory diversity, and (2) they do not aim to learn STL rule-compliance trajectories. The closest to our work to tackle traffic applications is CTG [2]. Thus, we chose CTG as the baseline and followed their closed-loop testing setup, which we explained in the updated Sec.~\ref{sec:exp-closed-loop}. Nevertheless, our approach serving as an add-up module could also be evaluated in a windowed fashion, with the potential to improve these baselines further. It will be an exciting exploration to combine our approach with the windowed policy to tackle other applications for future works.


\section{Responses to Reviewer-5 (Review355677)}
We are glad to see that our updated paper addresses your concerns about the initial submission. Thank you for helping us improve the paper.


\section{Responses to Reviewer-6 (Review355679)}
We appreciate the constructive feedback and the opportunity to make further improvements to our work.
Thanks for your suggestion. Below, we have provided detailed responses to address your questions and comments.

\subsection{About diverse trajectories generation}
We agree that CTG can also implicitly generate diverse policy (it is also the best baseline that can generate the most diverse trajectories). In contrast, our approach inherits the implicit diversity resulting from the diffusion model and further explicitly improves the diversity and the quality of the generated trajectories using RefineNet. We reflect this claim in the last paragraph of Sec.~\ref{sec:intro}.

\subsection{The human-robot interaction experiment}
Thanks for showing interest in our new conduct human-robot interaction experiment. We are not saying that our approach generates close to ``original human demonstrations". We only claim that our generated trajectories are the closest to the oracle (\textit{Traj. Opt.}). It is not our objective to perform trajectory prediction on the original demonstration data. We conducted this experiment following Reviewer 3 suggestion (``consider some more environments maybe even beyond self-driving to make it a stronger paper.") Thus, we are leaning towards keeping this experiment in the final paper.

\subsection{The training loss not reflecting the entropy}
Thanks for pointing it out. We explained why we are not directly optimizing entropy in the updated paper (above Eq(8)).

\subsection{Non-divese rule-compliance policy that discards the RefineNet output} We apologize for our misunderstanding and for not addressing your point in the initial submission. Hypothetically, you are correct that if the policy could find a very non-diverse behavior per mode that is rule-compliant, RefineNet will have no further improvement on diversity. We have addressed this limitation in Sec.~\ref{sec:conclusion} accordingly. However, in reality, for the training on NuScenes and human-robot encounter cases, the policy tends to have a very low rule compliance rate (unless the guidance step is triggered in the inference stage), which is also one of the motivations (as we mentioned in footnote 3 on page 4) for us to design the RefineNet to improve the trajectory quality. Even if the policy learns to generate non-diverse but rule-compliant trajectories under some extreme circumstances, we could then change the inference logic to be: choose the RefineNet output whenever the RefineNet trajectories are rule-compliant (while keeping the training logic the same as before). A more mathematical representation will be:
\begin{equation}
    \tau_{final}' = \tau_d + \mathds{1}\{\rho(\tau_d+g_r(z,\gamma,\tau_d),0,\Psi(\gamma,c))>0\}g_r(z,\gamma,\tau_d)
\end{equation}. Another way of tackling this is to generate the final solution in a probabilistic way based on $X\tau_{final} + (1-X)\tau_{final}'$ where $X\sim\text{Bernoulli}(0.5)$. We hope this addresses your concern.

\section{Responses to Reviewer-7 (Review355681)}

Thanks for your feedback. We apologize for not showing the changes in the highlighted colors. Our changes are not only in the presentation; we also conducted some ablation studies and designed a new experiment regarding a human-robot encounter scenario. We hope these added experiments make the paper stronger. 

We admit our proposed method is not guaranteed to generate rule-compliant trajectories. The guarantee is generally hard to satisfy for the problems with nonlinear dynamic systems and non-convex, nonlinear specifications. There are some additional post-processing steps that could add guarantees to the whole pipeline, such as the sampling-based backup policy used in [3] or using Control Barrier Functions (CBF) to ensure at least the safety concept in the specifications as in [4]. However, these are beyond the scope of this paper. 


\section{List of changes}
\begin{enumerate}
    \item Added Diffusion Policy [1] into reference, updated Sec.~\ref{sec:intro} and Sec.~\ref{sec:related} accordingly.
    \item Updated the rationale of choosing MPC rather than windowed policy for the closed-loop testing in Sec.~\ref{sec:exp-closed-loop}. 
    \item Updated the summary in Sec.~\ref{sec:intro}.
    \item Explained why we optimize for DPP loss rather than optimizing entropy directly in Sec.~\ref{sec:method-e}.
    \item Mentioned limitations about in Sec.~\ref{sec:conclusion}. 
    \item Other minor changes to fit the 8-page limit.
\end{enumerate}


\section*{References:}
% diffusion policy

\indent 1. Chi, C., et al. (2023). Diffusion policy: Visuomotor policy learning via action diffusion. Robotics: Science and Systems 2023
% 

2. Zhong, Z., Rempe, D., Xu, D., Chen, Y., Veer, S., Che, T., ... \& Pavone, M. (2023, May). Guided conditional diffusion for controllable traffic simulation. In 2023 IEEE International Conference on Robotics and Automation (ICRA) (pp. 3560-3566). IEEE.

3. Meng, Y., \& Fan, C. (2023). Signal temporal logic neural predictive control. IEEE Robotics and Automation Letters. 

4. Liu, W., Mehdipour, N., \& Belta, C. (2021). Recurrent neural network controllers for signal temporal logic specifications subject to safety constraints. IEEE Control Systems Letters, 6, 91-96.

==> rebuttal/zz_post_acceptance2.tex <==
\newpage
\onecolumn

\setcounter{equation}{0}
\setcounter{section}{0}
\titleformat{\section}{\large\raggedright}{\thesection}{1em}{}
\begin{center}
\LARGE{Statement of changes}
\end{center}

% \doublespacing
\linespread{2}

\vspace{2em}

% \red{make it spreaded}
We thank the editor of IEEE Robotics and Automation Letters (RA-L) for accepting our paper. This additional material addresses the remaining issue from the editor and reflects the changes in the manuscript. The updated content in the manuscript is written in \paca{``purple"}, and we appreciate your effort throughout the review process.


\section{Responses to the editor}

Thanks for your comment. We conducted a thorough review of the papers and found that only Diffusion Policy [1] and Motion Primitive Diffusion (MPD) [2] use a windowed policy, whereas BESO [3] predicts just one action based on goals and historical observations. 

MPD [2] predicts 12 timesteps (each timestep is 0.1s) of ``actions" at each planning step and then interacts with the environment (at a higher frequency) using the motion primitives resulting from these actions to enter the next planning step. We check their implementation and dataset in \url{https://scheiklp.github.io/movement-primitive-diffusion/} and the average data length for ``bimanual\_tissue\_manipulation\_train" split is 47.34, which is approximately 1/4 of the length as their prediction horizon. Besides, the paper mentions that \textit{``We focus on action sequences of length $1<n<N$ instead of single actions or full trajectories to balance compounding errors and online adaptability in real-world scenarios."} so they are not predicting the entire trajectory, and the main difference from the Diffusion Policy is that MPD has a motion primitive mechanism to further accurately decode the denoised ``actions" to fine-grained high-frequency action sequence.

BESO [3] is a goal-conditioned imitation learning approach using a Causal-Transformer architecture to perform action prediction. As mentioned in the paper, \textit{``During training, the denoised actions are inferred for all timesteps in the input series, yet only the last predicted action is utilized for inference."} Therefore, BESO is not a windowed policy method, and the reason we don't do action prediction is that our STL is defined on the trajectory level. And we don't adapt the goal-condition mechanism because the STL cannot be fully conveyed by just a few goal states (for example, if our specification is to ``always stay close to the centerline within 1.5 meters and eventually change to the left lane", this cannot be simply represented by just a few states.).

We agree that our first author's replies were better to fit in the context to explain why we chose MPC over windowed policy, and we updated the explanation in the footnote in Sec.~\ref{sec:exp-closed-loop}. We also added both BESO and MPD in Sec.~\ref{sec:related} to acknowledge their contribution.

% In BESO the goal is defined as a short sequence of states, whereas in our paper the specification can be treated as a ``goal" but may not be able to be fully conveyed by just using a short sequence of states: for example, if our specification is to ``always stay close to the centerline within 1.5 meter and eventually change to the left lane", this cannot be simply represented by just a few states. Besides, the specification is evaluated on a trajectory level, not just on the action level, so we do not consider


% From their config file in , we can know that the MPD predicts 12 timesteps of actions, and perform 12 steps into environment, with a replanning-frequency at every 12 steps. and their testing horizon is . So in that sense, they are still generating short sequence of action policies similar to 

% BESO is only goal-conditioned policy, with goals needed to specified for the rules. The goals are states, not in our case , we need to specify the STL rules (which does not directly reflect in).

% Actually the diffusion policy, BESO and MPD are representing different mechanisms. (though they can compare to each other; but why we cannot compare to them)

% The BESO paper also just uses one action in the inference, as they show in the paper "During training, the denoised actions are inferred for all timesteps in the input series, yet only the last predicted action is utilized for inference.". The difference is that they use goal-condition and use history observations for the transformer, whereas we just rely on the current state observation, and we use STL specification.

% The MPD paper does predict a sequence of actions for inference, but they are not using the whole trajectory for the inference, as they show in the paper "We focus on action sequences of length 1 < n < N instead of single actions or full trajectories to balance compounding errors and online adaptability in real-world scenarios.".

% For that saying, 


\section{List of changes}
\begin{enumerate}
    \item Added BESO [2] and MDP [2] into reference, updated  Sec.~\ref{sec:related} accordingly.
    \item Updated the rationale of choosing MPC rather than windowed policy for the closed-loop testing in Sec.~\ref{sec:exp-closed-loop}. 
    \item Other minor changes to fit the 8-page limit.
\end{enumerate}


\section*{References:}
% diffusion policy

\indent 1. Chi, C., et al. (2023). Diffusion policy: Visuomotor policy learning via action diffusion. Robotics: Science and Systems 2023
% 

2. Scheikl, Paul Maria, et al. "Movement primitive diffusion: Learning gentle robotic manipulation of deformable objects." IEEE Robotics and Automation Letters (2024).

3. Reuss, M., Li, M., Jia, X., \& Lioutikov, R. (2023). Goal-conditioned imitation learning using score-based diffusion policies. arXiv preprint arXiv:2304.02532.



==> rebuttal/zz_statement_of_changes.tex <==
\newpage
\onecolumn

\setcounter{equation}{0}
\setcounter{section}{0}
\titleformat{\section}{\large\raggedright}{\thesection}{1em}{}
\begin{center}
% \Huge{Statement of Changes}
\LARGE{Statement of Changes}
\end{center}


\newcommand{\ablationexp}{We have conducted ablation studies to show the importance of each component/loss in our learning framework and present the result in the updated Table~\ref{tab:open-loop}. Here ``\ournor" does not use RefineNet and only uses DDPM, ``\ourstl" replaces the diversity loss used in our method with a negative STL robustness score introduced in [5] as the loss function to train the RefineNet. Without using RefineNet, the performance is similar to the ``DDPM" method, where the gains ($14\%$ in success rate, $56\%$ increase in compliance, and $71\%$ in valid area) result from the ensemble of the diffusion model outputs generated from the last five denoising steps (we also added this explanation in Sec.~\ref{sec:method-e}), but the performance is much lower than ``Ours" (especially the rule compliance rate, valid area, and entropy). With the STL loss used, ``\ourstl" can achieve a high rule compliance rate, with a $47-188\%$ increase in the diversity measure compared to ``\ournor". Further using the diversity loss, ``Ours" achieves a $19-22\%$ improvement in the trajectory diversity. And finally with the guidance used, ``Ours+guidance" generates the most diverse trajectories, at the cost of 4X longer inference time compared to ``Ours". We can see that adding the RefineNet and training it with a diversity loss significantly improves the diversity and rule compliance rate of the trajectories, which indicates the importance of our design. These descriptions have also been added to in Sec.~\ref{sec:exp-open-loop}.
}

\newcommand{\ctgtimeexplain}{The reason that the other diffusion models like CTG [4] are significantly slower than our approach is that the CTG model computes guidance at every denoising step (as mentioned in [1]), whereas our approach only computes the guidance in a subset of denoising steps. Computing the guidance requires running gradient descent, which takes up the majority of the runtime (the total time is almost linear to the number of steps that compute the guidance). We found it sufficient to compute the guidance at the end: the total diffusion steps is 100 and we only compute guidance in the last five steps. Hence, we have a 16X speed-up compared to the CTG [4] (because we also have a RefineNet). Running more guidance steps will certainly improve our algorithm's performance in diversity and rule compliance but will also increase latency. We just show a sweet point to show that our approach can reach higher performance with much less computation time. We have also updated the main paper to illustrate this fact.}

% \doublespacing
\linespread{2}

\vspace{2em}

% \red{make it spreaded}
We thank all reviewers and the editor of IEEE Robotics and Automation Letters (RA-L) for reviewing our paper. Your valuable feedback has been instrumental in enhancing the quality and contribution of our work. We have carefully addressed the reviewers' concerns, making corresponding changes to the manuscript and incorporating additional experimental results to strengthen the novelty and impact of our research. \rbt{The modified content has been written in the ``Maroon" color same as this sentence.} We appreciate your time and consideration throughout this review process and eagerly await the final decision on our submission.
\section{Responses to the editor}
Thanks for your summarization. Per reviewer requests, we added extra experiments (human-robot encounter scenarios) and ablation studies (in Table~\ref{tab:open-loop}) to strengthen our algorithm design and to support our updated contributions (in the last paragraph of Sec.~\ref{sec:intro}). We have clarified the concepts regarding STL, DDPM and TrajOpt in Sec.~\ref{sec:prelim}, Sec.~\ref{sec:tech} and Sec.~\ref{sec:exp}, and we have cleared the typos mentioned by the reviewers. Overall, we think our paper has shown certain contributions qualified for RA-L publishing.
% Thanks for your summarization. Per reviewer requests, we added extra experiments and baselines, and also run extra random seeds for better variance. Regarding the novelty/contribution, in this work, we show that it is possible to learn a neural network controller to generate trajectories to satisfy a wide range of STL specifications. We also demonstrate the validity of our method on a broad spectrum of experiments, ranging from car and ship dynamics to robot arms and with different complexities in the STL specification. Besides, we conduct thorough comparisons and ablation studies. Thus overall, we think our paper has shown certain contributions qualified for RA-L publishing.

\section{Responses to Reviewer-1 (Review339255)}
% Thanks for your suggestion. We have added the requested baselines (three MBRL baselines) and experiments (robot manipulator) and updated the paper content.

Thanks for your suggestion. As suggested, we have corrected the terms for DDPM and other abbreviations and conducted further ablation studies for our proposed model design. In the updated submission, we illustrate the effort needed for STL calibration in Sec.~\ref{sec:tech}, and we added context in Sec.~\ref{sec:exp} to explain why our model is faster than the CTG method [4] (DDPM with guidance).

\subsection{Ablation for model designs} \ablationexp
% In high-level summary, our learning framework consists of a DDPM and a RefineNet, where the DDPM emsembled outpu: we first train the DDPM using the diffusion loss in Eq.~\eqref{eq:diffusion-loss}, and then keep the DDPM model parameters fixed, and further train the RefineNet using the loss in Eq.~\eqref{eq:diversity-loss}. 

\subsection{Runtime difference between other diffusion models and ours} \ctgtimeexplain

\subsection{Effort and details for STL calibration} Thanks for pointing it out. We have added the limitation of STL calibration in Sec.~\ref{sec:conclusion}. In fact, all the baselines we compare in Table~\ref{tab:open-loop} use the STL calibration (as they all need to have STL parameters as their input), and most of them used augmented data in training (where the ``Augmentation" column is marked as ``Yes"). Compared to the methods (``VAE", ``DDPM") that do not use augmented data, the ones (``VAE", ``DDPM") that use the augmented data can achieve a higher diversity measure (up to $95\%$ increase in ``Valid area" and up to $23\%$ increase in ``Entropy"). The reason that we need to use STL calibrated parameters as input for all the baselines is that we need to test their controllability (given a set of STL parameters, generate diverse and rule-compliant trajectories for these parameters), and the evaluation metrics ``Compliance", ``Valid area" and ``Entropy" all rely on the correctness of the trajectory satisfying the parametrized STL formula. The limitation of our approach is the manual laboring effort for the high-level behavior and heuristic-based design to calibrate the STL parameters. The high-level behavior labeling costs a week in annotation tool design and testing, and four days for a student to label the data on the NuScenes dataset. The STL parameter calibration process design costs less than a day, and the calibration process can run on the fly in the training/inference stages without much overhead. To reduce the design/calibration effort for the other researchers, we mention in the paper that we would like to release our annotation tool and the labels for the data after the paper gets accepted.


\section{Responses to Reviewer-2 (Review339257)}
Thanks for the detailed constructive feedback. We have addressed all your suggestions (rectifying the contribution, rephrasing the preliminary section (Sec.~\ref{sec:prelim}), adding ablation studies, explaining the STL parameter selection rationale for the closed-loop test, and correcting the typos) and made corresponding updates in the paper. Here are some answers to your questions.

\subsection{About contributions} Thanks for your suggestion, and we have updated our contribution accordingly in Sec.~\ref{sec:contribution}. Our main contribution is to use a parametrized-STL formulation to generate diverse and controllable trajectories that are rule-compliant. While CTG [4] can also generate controllable and rule-compliant trajectories, they do not address the trajectory-level ``diversity" but more on the rule-level ``diversity." (their approach can handle diverse STL rules on the fly using the guidance, but they don't tackle the problem of generating diverse trajectories for one given STL rule.) Our approach encourages the trajectories satisfying the same STL rule to be as diverse as possible via data augmentation and the RefineNet. We can also handle multiple STL rules like CTG [4] does, which is an advantage of using diffusion models for policy generation.

\subsection{Rules \texorpdfstring{$\phi_4$}{} and \texorpdfstring{$\phi_5$}{}: ``eventually" and ``always" being in the same time interval} Thanks for pointing it out, and we have added a footnote in Sec.~\ref{sec:calibration} to explain this complex syntax. In short, this should be read as: ``eventually" and then ``always", which can be interpreted as ``after some time steps, the signal should always satisfy the constraints (e.g., distance constraint in $\phi_4^H$ and angle constraint in $\phi_5^H$)." The time intervals for STL temporal operators work in a relative fashion: the ``[0, T]" for the ``always" operator is actually set after a certain time step in ``[0, T]" for the ``eventually" operator. Mathematically, the semantic for $\phi_5^H$ is: $\exists t\in[0,T], s.t. \forall t'\in[t, t+T], |Angle(s(t'),Q_h)|\leq \theta_{max}$. In this paper, we used a truncated time window, so the right interval for $t'$ actually becomes $min(t+T, T)=T$. A similar expression can be derived for $\phi_4^H$.

\subsection{The diversity concept in our paper} We have updated our paper accordingly to better explain the ``diversity" concept. In our work, diversity means the different policies an agent can generate in a certain scenario. The richness in the diverse trajectory set comes from three levels: (1) different discrete high-level decisions (2) different continuous STL parameters and (3) different trajectories for one high-level decision and one set of STL parameters. While we encode all these three aspects in generating diverse behaviors, the main novelty algorithm-wise is mainly from the third aspect. Multi-modality distribution could also happen at this level of diversity (imagine if a robot needs to avoid an obstacle in the scene and might have different routes to perform the task). We do not directly choose entropy as a loss term to guide the RefineNet because this term is hard to optimize (approximating the entropy requires state space discretization, which makes gradient-based optimization difficult to proceed with). Thus, we choose the loss mentioned in [6] to improve the diversity.

\subsection{Ablation for the RefineNet} \ablationexp 

\subsection{Compared to windowed, closed-loop control with diffusion models} These methods [1,2,3] mainly work in the robot manipulation domain, where the task horizon is long and the environment is relatively static. The main challenge in our cases (driving scenarios) is that the environment can change suddenly during the planning process (a new neighbor vehicle emerges, lane changes, etc). The windowed, closed-loop planning used in [1,2,3] might not be able to react to these changes by default, and a mechanism to detect the environment change and trigger the replanning process is needed. While our MPC-style planning design might take a longer time to plan for every step, our approach is reactive to these changes and can respond accordingly.

\subsection{Runtime details and runtime comparison between CTG and our method} The runtime of 0.4 seconds for our method mainly resulted from the usage of the guidance during the DDPM denoising steps. The time difference (0.379-0.055=0.324 seconds, as shown in Table~\ref{tab:closed-loop}) between ``Ours+guidance" and ``Ours" is the runtime for using the guidance. The 17X and 24X faster runtime compared to CTG [4] is not a typo or implementation error. %It is mainly because ``our+guidance" computes fewer guidance steps than CTG does. 
\ctgtimeexplain 

\section{Responses to Reviewer-3 (Review339259)}
Thanks for recognizing our paper's values. We appreciate your suggestions and have conducted a new evaluation under the human-robot encounters scenario to further strengthen our paper. Besides, we have updated the paper to explain the relationship between RefineNet and other constrained-based diffusion models. Here are some answers to your questions.

\subsection{Expressiveness about the parametrized-STL formulation} In our paper, we demonstrate the fast vs slow driving patterns in Fig.~\ref{fig:diverse-demo}, where the speed limit is controlled by the continuous STL parameters. While we admit there exist some limitations for this approach to model more types of behaviors at the current stage, this is not because of the formulation of STL. Rather, it is more about how to collect and cluster trajectories/demonstrations into different categories and what continuous properties we want to encode in the STL formulas.

\subsection{Evaluation for human-robot encounter scenarios} We have conducted a new experiment to demonstrate how our approach can generate diverse
human behaviors under human-robot encounter scenarios. The details and results are in Sec.~\ref{sec:exp-hri}. We consider the scenario introduced in [7], where the STL rule for
the human is to reach the goal while avoiding collision with the incoming robot. In [7], they collected 1000 trajectories from 50 recruited participants on the Amazon Mechanical Turk (AMT) platform. These trajectories are long and reveal a bi-modal distribution. We choose 80-time steps as the cut-off length, as most of the trajectories will halt afterward. We choose collision thresholds as the STL parameters and calibrate them on these trajectories. The dataset is further augmented via the method in Sec.~\ref{sec:calibration}. We train our method and baselines on the augmented dataset to compare their open-loop trajectory prediction performance. The results in Table~\ref{tab:rbt-hri-open-loop} show that ``Ours+guidance" achieves the highest diversity measure (``Area" and ``Entropy") among all learning methods, reaching the most close-to-oracle (\textit{Traj. Opt.}) performance, while using only 1/35X of the time. ``Ours+guidance" gets  $24 \sim 38\%$ improvement over CTG~\cite{zhong2023guided} in rule-compliance rate and diversity, being 7.7X faster in inference speed. Visualizations from Fig.~\ref{fig:rbt-hri} show that the trajectory distribution of Ours\textsubscript{G} (Ours+guidance) is close to the oracle. These results show the advantage of our approach in generating diverse rule-compliant behaviors.


\subsection{Guarantees of our method and adapt to other diffusion models} 
% It is correct that our method first trains the DDPM via learning from demonstrations (which are generated from gradient-based optimization with an STL-related loss), and after that, a RefineNet is trained to correct the trajectories generated by the DDPM if they violate the STL constraints. 
The DDPM in our method may not be able to ``learn to solve STL problems", as reflected by the low rule-compliance rate from ``DDPM" and `\ournor" baselines in Table~\ref{tab:open-loop}. Therefore, we have designed the RefineNet to improve the rule-compliance rate and diversity of the trajectories generated by the DDPM (which is also testified in Table~\ref{tab:open-loop}). We acknowledge in Sec.~\ref{sec:conclusion} that one of our limitations is the lack of guarantees (even using the RefineNet). However, this can be tackled by using a backup policy (using sampling-based methods or MILP solvers) when our approach fails. Besides, we have demonstrated the possibility of integrating our method with diffusion models which add constraints in the sampling process (the ``Ours+guidance" approach in Table~\ref{tab:open-loop},~\ref{tab:closed-loop}~\ref{tab:rbt-hri-open-loop}), and doing this will improve the quality and diversity of the trajectories compared to ``Ours", but at a cost of much longer runtime. Since our approach does not have any restriction on the forms of the diffusion models, it could be easily adapted to other advanced diffusion models without extra effort.

\section{List of Changes}
\begin{enumerate}
    \item Conduct ablation study and appended the results in Table~\ref{tab:open-loop} to illustrate the impact of each individual component (and loss) in our framework.
    \item Conduct a new experiment on human-robot encountering scenarios and present both quantitative and qualitative results in Sec.~\ref{sec:exp-hri}.
    \item Added computation time for the Trajectory Optimization method (``\textit{Traj. Opt.}") in Table~\ref{tab:open-loop}.
    \item Added footnote in Sec.~\ref{sec:intro} to explain what does the ``diversity" mean in our context.
    \item Corrected and unified the full name and the description for DDPM in Sec.~\ref{sec:intro}, Sec.~\ref{sec:tech}, and Sec.~\ref{sec:exp}. Removed ``Diffusion learning" term in Sec.~\ref{sec:intro}. Capitalized the term ``diffusion models".
    \item Corrected the typos (an scene $\to$ a scene; doesn't $\to$ does not).
    \item Changed the ``Traj. Opt. augmented dataset" to ``augmented dataset" in Sec.~\ref{sec:exp}.
    \item Simplified and revised Sec.~\ref{sec:prelim} for easier understanding.
    \item Unified the symbols used for the diversity measure.
    \item Revised the lane variable description in the scene model section of Sec.~\ref{sec:sys-model} to be more informative.
    \item Removed the bracket in Eq~\eqref{eq:stl_formula} for better understanding.
    \item Explained the constraint of "Eventually Always ..." for $\phi_5^H$ in the footnote for Sec.~\ref{sec:sys-model}.     
    \item Other minor changes per reviewer's request or to fit the  8-page limit.
\end{enumerate}


\section*{References:}
% diffusion policy

\indent 1. Chi, C., et al. (2023). Diffusion policy: Visuomotor policy learning via action diffusion. Robotics: Science and Systems 2023
% 

\indent 2. Reuss, M., \& Lioutikov, R. (2023). Goal-Conditioned Imitation Learning using Score-based Diffusion Policies. Robotics: Science and Systems 2023

% 
3. Scheikl, P. M., et al. (2024). Movement primitive diffusion: Learning gentle robotic manipulation of deformable objects. IEEE Robotics and Automation Letters.

% CTG
4. Zhong, Z., Rempe, D., Xu, D., Chen, Y., Veer, S., Che, T., ... \& Pavone, M. (2023, May). Guided conditional diffusion for controllable traffic simulation. In 2023 IEEE International Conference on Robotics and Automation (ICRA) (pp. 3560-3566). IEEE.

% semi
5. Leung, K., \& Pavone, M. (2022, June). Semi-supervised trajectory-feedback controller synthesis for signal temporal logic specifications. In 2022 American Control Conference (ACC) (pp. 178-185). IEEE.

% diverse
6. Yuan, Y., \& Kitani, K. (2019). Diverse trajectory forecasting with determinantal point processes. arXiv preprint arXiv:1907.04967.

7. Linard, A., Torre, I., Steen, A., Leite, I., \& Tumova, J. (2021, September). Formalizing trajectories in human-robot encounters via probabilistic stl inference. In 2021 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS) (pp. 9857-9862). IEEE.
